The CMS Fast Beam Condition Monitor for HL-LHC

The high-luminosity upgrade of the LHC brings unprecedented requirements for real-time and precision bunch-by-bunch online luminosity measurement and beam-induced background monitoring. A key component of the CMS Beam Radiation, Instrumentation and Luminosity system is a stand-alone luminometer, the Fast Beam Condition Monitor (FBCM), which is fully independent from the CMS central trigger and data acquisition services and able to operate at all times with a triggerless readout. FBCM utilizes a dedicated front-end application-specific integrated circuit (ASIC) to amplify the signals from CO$_2$-cooled silicon-pad sensors with a timing resolution of a few nanoseconds, which enables the measurement of the beam-induced background. FBCM uses a modular design with two half-disks of twelve modules at each end of CMS, with four service modules placed close to the outer edge to reduce radiation-induced aging. The electronics system design adapts several components from the CMS Tracker for power, control and read-out functionalities. The dedicated FBCM23 ASIC contains six channels and adjustable shaping time to optimize the noise with regards to sensor leakage current. Each ASIC channel outputs a single binary high-speed asynchronous signal carrying time-of-arrival and time-over-threshold information. The chip output signal is digitized, encoded and sent via a radiation-hard gigabit transceiver and an optical link to the back-end electronics for analysis. This paper reports on the updated design of the FBCM detector and the ongoing testing program.

==> tex/simulation.tex <==
\section{TEMPORARY --- Simulation}
\label{sec:sim}

\textcolor{red}{[Who was writing this section? Text can be partly re-purposed in the introduction part, but plots can not be used in the paper, as they are not approved. If you want to approve them, the last possibility will be to prepare full presentation with plots, captions, all relevant results for DPG session on the 5th of December. And even in this case it might be not possible to be ready to Run Coordination approval before the deadline for submission on the 11th of December. ]}

Full CMSSW simulations, incorporating an appropriate model for the front-end electronics, were conducted to evaluate the performance of the proposed system and optimize some of its parameters. These simulations were carried out in a private branch of CMSSW\_ 11\_2\_0\_pre10, which included the FBCM geometry, detector simulation using GEANT4, and a customized digitizer.


\subsection{Geometry}
The geometry of the FBCM simulation consists of 67,000 sensors with an area of $2.89 mm^2$, positioned on the FBCM disc from a radius of 8.5cm up to a radius of 22cm. In this study, we consider two kinds of sensors based on their thickness: one with a thickness of 290 micrometers and the other with a thickness of 150 micrometers. Therefore, we have two geometries; one with 67,000 sensors, an area of $2.89 mm^2$, and a thickness of 290 micrometers, and the other with the same area but a thickness of 150 micrometers. 

Note: The real FBCM consists of only 336 sensors. The geometry studied in the current analysis was designed to investigate the behavior of the sensors at different radii.
\subsection{Implementation of ASIC details}
The FBCM digitizer replicates the functionality of the front-end ASIC and plays a crucial role in shaping the linearity behavior. For this study, we implemented a fixed-threshold discriminator with time walk compensation. The FBCM digitizer also benefits from simulating five subsequent bunches simultaneously. This feature is crucial for addressing the impacts of out-of-time bunches and prolonged pulses that might extend from preceding bunch slots to the current one. However, the effects of afterglow and albedo are not considered in the FBCM digitizer at its current stage. Additionally, the current version of the digitizer lacks support for pulse truncation at 25 ns for long pulses with Time over Threshold (ToT) greater than 25 ns, as anticipated for the Phase-2 FBCM front-end ASIC.

\subsection{silicon sensors}

Silicon-pad sensors are a promising option for luminosity measurement, since they are easy to produce, can be designed to have a good signal-to-noise ratio, and will benefit from advances in cooling technology foreseen for CMS for Phase-2. Technological choices for the silicon sensors, in terms of radiation hardness, profit from the research and development experience gathered by the Tracker~\cite{CERN-LHCC-2017-009} and HGCAL~\cite{CERN-LHCC-2017-023} projects.
\subsubsection{amplitudes}
\subsection{results}
The linearity of FBCM measurements, crucial for luminosity measurement, was assessed in CMSSW as a function of average pileup. To achieve this, the mean number of observable hits per sensor per bunch crossing (BX), denoted by the mean ($\lambda$) of a Poisson distribution, was estimated using the zero-counting approach. To evaluate the deviation from linearity(Fig. \ref{fig:overall}, middle) the values of $\lambda$ as a function of pileup were fitted with a straight line, covering only the range up to PU = 1.5 (i.e., the simulations at PU = 0.5, 1, 1.5), and are displayed in Fig. \ref{fig:overall} on the left. The residuals with respect to the fit were then calculated at higher PU values.

To investigate the statistical precision of the detector, the relative uncertainty ($\epsilon_{ZC}$) in the zero-counting approach can be calculated using Equation \ref{err}. Here, M represents the total number of samples collected by the detector for one bunch location (i.e., the product of the number of sensors and the number of crossings which is the $f_{rev} = 11245.5 Hz$) during the integration time of $\tau$ = 1 s:

\begin{equation}
    \epsilon_{ZC} = \frac{\sqrt{e^{\lambda}-1}}{\lambda \sqrt{M}}\label{err}
\end{equation}



\begin{figure}[ht]
\centering
\includegraphics[width=1.\textwidth]{./fig/simulation/last}
%\includegraphics[width=0.32\textwidth]{./figs/dev4}
%\includegraphics[width=0.32\textwidth]{./figs/uncertainty}
 \caption{The average number of hits per bunch crossing (left), the deviation from linearity with total uncertainty  (center), and the statistical uncertainty in the rate (right) were evaluated at pileup 200 with an integration period of 1 second for 336 sensors. Each sensor has a size of 2.89 mm², and there are two thicknesses: one is 150 micrometers, and the other is 290 micrometers. The sensors are positioned at 
$r\approx 14.5 cm.$}
  \label{fig:overall}
\end{figure}


